Leveraging Domain Knowledge at Inference Time for LLM Translation: Retrieval versus Generation

While large language models (LLMs) have been increasingly adopted for machine translation (MT), their performance for specialist domains such as medicine and law remains an open challenge. Prior work has shown that LLMs can be domain-adapted at test-time by retrieving targeted few-shot demonstrations or terminologies for inclusion in the prompt. Meanwhile, for general-purpose LLM MT, recent studies have found some success in generating similarly useful domain knowledge from an LLM itself, prior to translation. Our work studies domain-adapted MT with LLMs through a careful prompting setup, finding that demonstrations consistently outperform terminology, and retrieval consistently outperforms generation. We find that generating demonstrations with weaker models can close the gap with larger model's zero-shot performance. Given the effectiveness of demonstrations, we perform detailed analyses to understand their value. We find that domain-specificity is particularly important, and that the popular multi-domain benchmark is testing adaptation to a particular writing style more so than to a specific domain.

==> tables/main_table_raw.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l|rrr|rrr|rrr}
               & \multicolumn{3}{c|}{\textbf{Gemini 1.5 Pro}} & \multicolumn{3}{c|}{\textbf{Gemma-2 27B IT}} & \multicolumn{3}{c}{\textbf{Tan et al., 2024}}                 \\
\textbf{strategy} & \textbf{law} & \textbf{med.} & \textbf{koran} & \textbf{law} & \textbf{med.} & \textbf{koran} & \textbf{law} & \textbf{med.} & \textbf{koran} \\
\hline
zero-shot                & 86.6                             & 88.2                                 & 76.3                               & 84.8                             & 85.2                                 & 75.1 & 84.4 & 86.8 & 75.1                               \\
\hline
retrieved terms & \textbf{86.9} & 88.5 & 74.9 & \textbf{85.9} & \textbf{87.8} & 74.6 & -- & -- & --\\
retrieved demos & \textbf{89.5} & \textbf{90.2} & \textbf{76.7} & \textbf{88.2} & \textbf{89.9} & \textbf{76.8} & 88.2 & 89.6 & 76.5 \\
generated terms                & 86.5                             & 87.8                                 & 76.2                               & 85.0                             & \textbf{87.4}                        & \textbf{76.3} & -- & -- & --\\
generated demos                 & \textbf{87.2}                    & \textbf{88.8}                        & \textbf{76.7}                      & \textbf{86.9}                    & \textbf{88.6}                        & \textbf{76.6} & -- & -- & --
\end{tabular}
\caption{Domain knowledge presented as demonstrations (demos) or terminology (terms), either \textit{retrieved} from external sources or \textit{generated} by the LLM. Reporting comet22 scores, with significant improvements over the zero-shot baseline bolded, and scores from \citet{tan-etal-2024-narrowing} provided for context. Demonstrations outperform terminology, and retrieval outperforms generation. Generation has larger effects for the smaller Gemma model. \label{tab:main_results}}
\end{table*}

